Private Aggregate Queries to Untrusted Databases

Private information retrieval (PIR), a privacy-preserving cryptographic tool, solves a simplified version of this problem by hiding the database item that a client accesses. Most PIR protocols require the client to know the exact row index of the intended database item, which cannot support the complicated aggregation-based statistical query in a similar setting. Some works in the PIR space contain keyword searching and SQL-like queries, but most need multiple interactions between the PIR client and PIR servers. Some schemes support searching SQL-like expressive queries in a single round but fail to enable aggregate queries. These schemes are the main focus of this paper. To bridge the gap, we have built a general-purpose novel information-theoretic PIR (IT-PIR) framework that permits a user to fetch the aggregated result, hiding all sensitive sections of the complex query from the hosting PIR server in a single round of interaction. In other words, the server will not know which records contribute to the aggregation. We then evaluate the feasibility of our protocol for both benchmarking and real-world application settings. For instance, in a complex aggregate query to the Twitter microblogging database of 1 million tweets, our protocol takes 0.014 seconds for a PIR server to generate the result when the user is interested in one of 3K user handles. In contrast, for a much-simplified task, not an aggregate but a positional query, Goldberg's regular IT-PIR (Oakland 2007) takes 1.13 seconds. For all possible user handles, 300K, it takes equal time compared to the regular IT-PIR. This example shows that complicated aggregate queries through our framework do not incur additional overhead if not less, compared to the conventional query.

==> macros.tex <==
\newcommand{\titletext}{Private Aggregate Queries to\\Untrusted Databases}
\newcommand{\keywordstext}{Private aggregate queries, Private information retrieval, Privacy-enhancing technology, Cryptography}% Applied c
% \newcommand{\figureref}[1]{Figure~\ref{#1}\xspace}
% \newcommand{\sectionref}[1]{Section~\ref{#1}\xspace}
% \newcommand{\tableref}[1]{Table~\ref{#1}\xspace}
% \newcommand{\customlstlisting}[1]{
% \begin{lstlisting}[
%             breaklines=true,
%            language=SQL,
%            showspaces=false,
%            basicstyle=\ttfamily,
%            numbers=left,
%            numberstyle=\tiny,
%            commentstyle=\color{gray}
%         ]
% #1
% \end{lstlisting}
% }

%%%%%%%%%%%%%% copied from syed's thesis %%%%%%%%%%%%%


\let\oldvec\vec
\renewcommand{\vec}[1]{\smash{\oldvec{\mathbf{#1}}}}
\DeclareSymbolFont{matha}{OML}{txmi}{b}{it}% txfonts
\DeclareMathSymbol{\varv}{\mathord}{matha}{118}
\newcommand{\vecF}{\vec{\rule[-.3\baselineskip]{0pt}{0.82\baselineskip}\smash{\scalebox{1}[0.95]{$\mathbf{F}$}}}} %changed from 0.3 to 0.45
% \newcommand{\vecF}{\vec{\rule[-.475\baselineskip]{0pt}{0.82\baselineskip}\smash{\scalebox{1}[0.95]{$\mathbf{F}$}}}}
\newcommand{\vecv}{\vec{\boldsymbol{\varv}}}
\newcommand{\vecQ}[1][\j]{\vec{\rule[-.475\baselineskip]{0pt}{0.82\baselineskip}\smash{\scalebox{1}[0.95]{$\mathbf{Q}$}}}_{\raisebox{0.1ex}{$\scriptstyle#1$}}}

\newcommand{\vecR}[1][\j]{\mkern-2mu\vec{\mkern2mu\rule[-.3\baselineskip]{0pt}{0.82\baselineskip}\smash{\scalebox{1}[0.95]{$\mathbf{R}$}}}_{\raisebox{0.1ex}{$\scriptstyle#1$}}}
%\newcommand{\plabel}[1]{\scalebox{0.88}[1]{\textls[-55]{$\scriptscriptstyle\mathtt{#1\mkern-2mu}$}}}
\newcommand{\plabel}[1]{\raisebox{0.1ex}{\scalebox{0.75}[1]{\textls[-50]{$\scriptscriptstyle\boldsymbol{\mathtt{#1\mkern-3mu}}$}}}}
\let\oldPi\Pi
\renewcommand{\Pi}[1][]{\oldPi_{\plabel{#1}}}

\newcommand{\p}{\mathpzc{p}}

\newcommand{\Eij}[1][i]{E_{\raisebox{0.25ex}{\smaller[0.5]$\scriptstyle\kern-0.25pt(\kern-0.5pt#1\kern-0.25pt,\kern-0.5ptj\kern-0.55pt)$}}}
\newcommand{\Dij}[1][i]{\D_{\raisebox{0.25ex}{\smaller[0.5]$\scriptstyle\kern-0.25pt(\kern-0.5pt#1\kern-0.25pt,j\kern-0.55pt)$}}}
\newcommand{\DIJ}[2]{\D_{\raisebox{0.25ex}{\smaller[0.5]$\scriptstyle\kern-0.25pt(\kern-0.5pt#1,\kern-0.5pt#2\kern-0.55pt)$}}}
\newcommand{\gij}[2]{g_{\raisebox{0.25ex}{\smaller[0.5]$\scriptstyle\kern-0.25pt(\kern-0.5pt#1\kern-0.25pt,\kern-0.5pt#2\kern-0.55pt)$}}(x)}
\newcommand{\Di}[1][i]{\mkern-2.5mu\vec{\mkern2.5mu\D}_{\raisebox{0.25ex}{\smaller[0.5]$\scriptstyle\kern-0.25pt#1$}}}
\newcommand{\f}[1][i]{f_{\raisebox{0.25ex}{\smaller[0.5]$\scriptstyle\kern-0.5pt#1$}}}

\newcommand{\Pik}[1][k]{\oldPi^{\raisebox{-0.2ex}{\smaller[0.5]$\scriptstyle\kern-0.25pt(\kern-0.2pt#1\kern-0.55pt)$}}}
\newcommand{\Pikij}[1][i]{\Pik_{\raisebox{0.25ex}{\smaller[0.5]$\scriptstyle\kern-0.25pt(\kern-0.5pt#1\kern-0.25pt,\kern-0.5ptj\kern-0.55pt)$}}}
\newcommand{\Piij}[1][i]{\oldPi_{\raisebox{0.25ex}{\smaller[0.5]$\scriptstyle\kern-0.25pt(\kern-0.5pt#1\kern-0.25pt,\kern-0.5ptj\kern-0.55pt)$}}}
\newcommand{\iq}{i_{\mkern-2mu\raisebox{0.2ex}{\scalebox{0.725}[0.875]{$\scriptscriptstyle q$}}}}
\newcommand{\iqq}[1][]{i_{\mkern-1.25mu\raisebox{0.15ex}{\scalebox{0.6}[0.8]{$\scriptscriptstyle Q_{#1}$}}}}
\newcommand{\ir}{i_{\mkern-2mu\raisebox{0.2ex}{\scalebox{0.7}[0.85]{$\scriptscriptstyle R$}}}}

\newcommand{\iQ}[1][]{i_{\mkern-2mu\raisebox{0.2ex}{\scalebox{0.85}[0.975]{$\scriptstyle Q_{#1}$}}}}
\newcommand{\iR}[1][]{i_{\mkern-3mu\raisebox{0.2ex}{\scalebox{0.95}[0.95]{$\scriptstyle R_{#1}$}}}}


\newcommand{\fvec}[1][\mkern4mu]{\smash{\mkern3mu\vec{\mkern-3mu\boldsymbol{f}}\mkern-4mu_{#1}}}
\newcommand{\dvec}[1][\mkern4mu]{\smash{\mkern3mu\vec{\mkern-3mu\boldsymbol{d}}\mkern-1mu_{#1}}}
\newcommand{\0}{\scalebox{0.9}{\kern0.25pt$\scriptstyle0$}}
\newcommand{\1}{\scalebox{0.9}{\kern0.25pt$\scriptstyle1$}}
\newcommand{\2}{\scalebox{0.9}{\kern0.25pt$\scriptstyle2$}}
\newcommand{\K}{m}
\newcommand{\D}{\scalebox{1}[0.95]{$\mathbf{D}$}}
\newcommand{\Du}[1][]{\mathbf{D}^{\scriptscriptstyle(\u)}_{\smash{\raisebox{0.15ex}{\smaller[0.5]$\scriptstyle\kern-0.25pt#1$}}}}
\newcommand{\Duu}[1]{\mathbf{D}^{\scriptscriptstyle(#1)}}
\newcommand{\DU}[1][]{\vec{\mathbf{D}}^{\scriptscriptstyle(\u)}_{\smash{\raisebox{0.15ex}{\smaller[0.5]$\scriptstyle\kern-0.25pt#1$}}}}
\newcommand{\DD}[1][]{\tilde{\mathbf{D}}_{\raisebox{0.25ex}{\smaller[1]$\scriptstyle\kern-0.25pt#1$}}}
\newcommand{\Piu}[1][\u]{\oldPi^{\scriptscriptstyle(#1)}}
%\newcommand{\q}{\mathchoice%
%{\scalebox{0.9}{$\mathpzc{q}$}}%
%{\scalebox{0.9}{$\mathpzc{q}$}}%
%{\scalebox{0.9}{$\scriptstyle\mkern-2mu\mathpzc{q}$}}%
%{\scalebox{0.9}{$\scriptscriptstyle\mkern-2mu\mathpzc{q}$}}}
\newcommand{\q}{q}
\let\aaa\r
\renewcommand{\aa}{\aaa{a}}
\let\r\relax\newcommand{\r}{\mathpzc{r}}
\let\s\relax\newcommand{\s}{\mathpzc{s}}
\let\t\relax\newcommand{\t}{\kern-0.15ex\mathpzc{t}}%\kern-0.15ex
\let\R\relax\newcommand{\R}{\mathcal{R}}
\let\n\relax\newcommand{\n}{\mathpzc{n}}
\let\m\relax\newcommand{\m}{\mathpzc{m}}
%\let\oldell\ell\renewcommand{\ell}{\oldell\kern0.15ex}
\let\u\relax\newcommand{\u}{\mkern-0.75mu\mathpzc{u}\mkern0.75mu}
\let\v\relax\newcommand{\v}{\mathpzc{v}}
\let\w\relax\newcommand{\w}{\mathpzc{w}}
\let\z\relax\newcommand{\z}{\mathpzc{z}}
\newcommand{\e}[1][i]{\vec{\boldsymbol{e}}_{\raisebox{0.125ex}{\smaller[1.5]$\scriptstyle\kern-1pt#1$}}}
\newcommand{\aggregate}[1][i]{\vec{\boldsymbol{e}}_{\raisebox{0.125ex}{\smaller[1.5]$\scriptstyle\kern-1pt#1$}}}
\newcommand{\setofindexes}{\mathcal{I}}
\newcommand{\secret}{\mathcal{S}}
\newcommand{\ru}{\inlinefrac{\r}{\u}}
%\newcommand{\ru}{\lceil\mkern-1.5mu\inlinefrac{\r}{\u}\mkern-1.5mu\rceil}
\newcommand{\Rell}{\lceil\mkern-1.5mu\inlinefrac{\R}{\ell}\mkern-1.5mu\rceil}
\newcommand{\rell}{\r\ell}
\newcommand{\ruell}{\lceil\inlinefrac{\rell}{\u}\rceil}

\newcommand{\Rn}{\lceil\mkern-1.5mu\inlinefrac{\R}{\n}\mkern-1.5mu\rceil}
\newcommand{\rn}{\r\n}
\newcommand{\run}{\lceil\inlinefrac{\rn}{\u}\rceil}


\newcommand{\rs}{\r\kern0.0075ex\s}
\newcommand{\ps}{\p\mkern1.1mu\s}
\newcommand{\qr}{\scalebox{1}[1.09]{$\q$}\kern0.0075ex\r}
\newcommand{\qs}{\scalebox{1}[1.09]{$\q$}\kern0.0075ex\s}
\newcommand{\qrs}{2\kern0.185ex\scalebox{1}[1.09]{$\q$}\kern0.0085ex\r\kern0.0075ex\s}
\newcommand{\tr}{\t\kern0.0075ex\r}
\newcommand{\tru}{\t\kern0.0075ex\ru}
\newcommand{\sell}{\s\kern0.025ex\ell}
\newcommand{\rbyr}{\mathchoice%
{\r\mathbin{\scalebox{0.9}{$\displaystyle\times$}}\r}%
{\r\mathbin{\scalebox{0.9}{$\textstyle\times$}}\r}%
{\r\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu\r}%
{\r\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu\r}}%

\newcommand{\kbyr}{\mathchoice%
{k\mkern1mu\mathbin{\scalebox{0.9}{$\displaystyle\times$}}\r}%
{k\mkern1mu\mathbin{\scalebox{0.9}{$\textstyle\times$}}\r}%
{\mkern0.75muk\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu\r}%
{k\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu\r}}%

\newcommand{\kbyrbyp}{\mathchoice%
{k\mkern1mu\mathbin{\scalebox{0.9}{$\displaystyle\times$}}\r\mkern1mu\mathbin{\scalebox{0.9}{$\displaystyle\times$}}\p}%
{k\mkern1mu\mathbin{\scalebox{0.9}{$\textstyle\times$}}\r\mkern1mu\mathbin{\scalebox{0.9}{$\textstyle\times$}}\p}%
{\mkern0.75muk\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu\r\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu\p}%
{k\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu\r\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu\p}}%

\newcommand{\pbyrbyk}{\mathchoice%
{\p\mkern1mu\mathbin{\scalebox{0.9}{$\displaystyle\times$}}\r\mkern1mu\mathbin{\scalebox{0.9}{$\displaystyle\times$}}k}%
{\p\mkern1mu\mathbin{\scalebox{0.9}{$\textstyle\times$}}\r\mkern1mu\mathbin{\scalebox{0.9}{$\textstyle\times$}}k}%
{\p\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu\r\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu k}%
{\p\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu\r\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu k}}%

\newcommand{\pbyr}{\mathchoice%
{\p\mkern1mu\mathbin{\scalebox{0.9}{$\displaystyle\times$}}\r}%
{\p\mkern1mu\mathbin{\scalebox{0.9}{$\textstyle\times$}}\r}%
{\p\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu\r}%
{\p\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu\r}}%

\newcommand{\pbyrbyu}{\mathchoice%
{\p\mkern1mu\mathbin{\scalebox{0.9}{$\displaystyle\times$}}\r\mkern1mu\mathbin{\scalebox{0.9}{$\displaystyle\times$}}\u}%
{\p\mkern1mu\mathbin{\scalebox{0.9}{$\textstyle\times$}}\r\mkern1mu\mathbin{\scalebox{0.9}{$\textstyle\times$}}\u}%
{\p\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu\r\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu\u}%
{\p\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu\r\\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu}}%



\newcommand{\rbys}{\mathchoice%
{\r\mathbin{\scalebox{0.9}{$\displaystyle\times$}}\s}%
{\r\mathbin{\scalebox{0.9}{$\textstyle\times$}}\s}%
{\r\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu\s}%
{\r\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu\s}}%
\newcommand{\qbyr}{\mathchoice%
{\scalebox{1}[1.09]{$\q$}\mathbin{\scalebox{0.9}{$\displaystyle\times$}}\r}%
{\scalebox{1}[1.09]{$\q$}\mathbin{\scalebox{0.9}{$\textstyle\times$}}\r}%
{\scalebox{1}[1.09]{$\q$}\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu\r}%
{\scalebox{1}[1.09]{$\q$}\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu\r}}%
\newcommand{\ubys}[1][\s]{\mathchoice%
{\u\mathbin{\scalebox{0.9}{$\displaystyle\times$}}#1}%
{\u\mathbin{\scalebox{0.9}{$\textstyle\times$}}#1}%
{\u\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu#1}%
{\u\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu#1}}%
\newcommand{\rubys}[1][\s]{\mathchoice%
{(\mkern-1.5mu\ru\mkern-1.5mu)\mathbin{\scalebox{0.9}{$\displaystyle\times$}}#1}%
{(\mkern-1.5mu\ru\mkern-1.5mu)\mathbin{\scalebox{0.9}{$\textstyle\times$}}#1}%
{(\mkern-1.5mu\ru\mkern-1.5mu)\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu#1}%
{(\mkern-1.5mu\ru\mkern-1.5mu)\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu#1}}%
\newcommand{\Rellbys}[1][\s]{\mathchoice%
{\Rell\mathbin{\scalebox{0.9}{$\displaystyle\times$}}#1}%
{\Rell\mathbin{\scalebox{0.9}{$\textstyle\times$}}#1}%
{\Rell\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu#1}%
{\Rell\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu#1}}%
\newcommand{\Rnbys}[1][\s]{\mathchoice%
{\Rn\mathbin{\scalebox{0.9}{$\displaystyle\times$}}#1}%
{\Rn\mathbin{\scalebox{0.9}{$\textstyle\times$}}#1}%
{\Rn\mkern1.7mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern1mu#1}%
{\Rn\mkern0.85mu\mathbin{\scalebox{0.85}{$\scriptstyle\times$}}\mkern0.5mu#1}}%


\DeclareRobustCommand{\fakeslu}{\tikz[baseline=(X.base),inner sep=0,outer sep=0] \node[xslant=0.15,scale=1.15] (X) {$\u\mkern-0.75mu$};}

\newcommand{\GF}{\mathbf{GF}}

\newcommand{\x}[1][\j]{x_
{\raisebox{0.1ex}{$\scriptstyle\mkern-0.5mu#1$}}}

\usepackage[outline]{contour}
\contourlength{1.5pt}

\newcommand{\twodots}{
\mathchoice
{\mathinner{\mkern-1mu\ldotp\mkern-1mu\ldotp\mkern-1mu}}
{\mathinner{\mkern-1mu\ldotp\mkern-1mu\ldotp\mkern-1mu}}
{\mathinner{\ldotp\ldotp}}
{\mathinner{\ldotp\ldotp}}
}
\newcommand{\ival}[2][1\mkern-1.5mu]{[#1\twodots#2]}
\newcommand{\transpose}[1]{\ensuremath{#1^{\mkern0.75mu\mathrm{T}}}}
\newcommand{\hammingweight}[1]{\mathrm{wt}(#1)}
\newcommand{\lastone}{h}

%%%%%%%% from henry.sty
% \newcommand{\cardinality}[2][]{\mathchoice
		% {\displaystyle\@abs[#1]{#2}}
		% {\textstyle\@abs[#1]{#2\kern-0.075ex}}
		% {\scriptstyle\@abs[#1]{#2\kern-0.15ex}}
		% {\scriptscriptstyle\@abs[#1]{#2\kern-0.12ex}}}
\newcommand{\numberofones}{\beta}
\newcommand{\rows}{\r}
\newcommand{\cols}{\s}
\newcommand{\bits}{\b}
\newcommand{\wordsize}{\w}
\newcommand{\coalition}{C}
\newcommand{\Query}[1][]{\ifstrempty{#1}{Q}{Q_{\raisebox{0.125ex}{\smaller[0.5]$\scriptstyle\mkern-1.5mu#1$}}}}



==> sec-aggregate-indexes.tex <==
\subsection{Indexes of aggregate queries}\label{s:expressive:aggregate}
In this section, we extend our indexes of queries techniques to support aggregate queries (only when the \emph{effective}\footnote{The database owner can create a snapshot of the original database with only numeric attributes and support aggregate queries them.} database has numerical attributes. We define the standard aggregate vector and simple index of aggregate queries next.

\begin{definition}\label{def:aggregatebasis}
Let $ \setofindexes $ be a set of indices and $2\leq\cardinality{\setofindexes}\leq\rows$. A \textsl{standard aggregate vector} $ \aggregate[\setofindexes]\in\F^{\rows}$ is a $(0,1)$-vector with an $1$ value at each index of the set $\setofindexes$.
\end{definition}

Note that when $\cardinality{\setofindexes}=1$, the standard aggregate vector turns into a standard basis vector. When we multiply a standard aggregate vector with a database, the following observation is straightforward according to simple linear algebra.

\begin{observation}
If $\aggregate[\setofindexes]$ is a standard aggregate vector and $\setofindexes$ is a set of indices $\set{i_1,\ldots,i_{\lastone}}$ where $\lastone=\hammingweight{\aggregate[\setofindexes]}$,\footnote{$i_{\lastone}$ is the position where the last $1$ is in the $\aggregate[\setofindexes]$, and $\lastone$ can be computed by the hamming weight, $\hammingweight{}$, of $\aggregate[\setofindexes]$.} then $\aggregate[\setofindexes]\cdot\D$ is a linear combination of particular records (indexed by $\setofindexes$) of the database.
\end{observation}

That means, $\aggregate[\setofindexes]\cdot\D=\Di[i_1]+\ldots+\Di[i_{\lastone}]\in\F^{\cols}$. We can accumulate such standard aggregate vectors and build an index of aggregate queries. Next, we define the simple index of aggregate queries in light of~\definitionref{def:simpleindex}.

\begin{definition}\label{def:simpleindex:aggregate}
An \textsl{simple index of aggregate queries} for a database $\D\in\F^{\rbys}$ is a $(0\mkern1mu,\mkern-1mu1)\mkern2mu$-matrix $\Pi\in\F^{\pbyr}$ in which each row is a \textsl{standard aggregate vector}.
\end{definition}

Now, we can quickly write the following observations\emdash

\begin{observation}\label{obs:permute:aggregate}
If $\e[]\in\F^{\r}$ is a standard basis vector and $\Pi\in\F^{\rbyr}$ is a simple index of aggregate queries, then $\e[]\cdot\Pi$ is a standard aggregate vector $\aggregate[\setofindexes]\in\F^{\rows}$, namely, $\aggregate[\setofindexes]=\e[]\cdot\Pi$.
\end{observation}

\begin{observation}\label{obs:pseudopermute:aggregate}
Let \smash{$\e[]\in\F^{\p}$} be a standard basic vector and let $\Pi\in\F^{\pbyr}$ be a simple index of aggregate queries with rank $\p \lastone$.
If \smash{$(\x[1],\vecQ[1]),\ldots,(\x[\ell],\vecQ[\ell])$} is a component-wise $(\t+1,\ell)\mkern2mu$-threshold sharing of $\e[]$, then \smash{$(\x[1],\vecQ[1]\cdot\Pi),\ldots,(\x[\ell],\vecQ[\ell]\cdot\Pi)$} is a component-wise $(\t+1,\ell)\mkern2mu$- and $(1,\ell)\mkern2mu$-threshold sharing of a standard aggregate vector $\aggregate[\setofindexes]\in\F^{\r}$; namely, of $\aggregate[\setofindexes]=\e[]\cdot\Pi$.\footnote{Specifically, the \smash{$\r-\p \lastone$} entries corresponding to all-\smash{$0$} columns in \smash{$\Pi$} are \smash{$(1,\ell)$}-threshold shares of \smash{$0$}; the remaining \smash{$\p \lastone$} entries are each \smash{$(\t+1,\ell)$}-threshold shares of either \smash{$0$} or \smash{$1$}.}
\end{observation}

We define the $t$-privacy for indexes of aggregate queries as follows\emdash

\begin{definition}\label{def:tprivacy:aggregate}
Let $\D\in\F^{\rbys}$ and let each $\oldPi_1,\ldots,\oldPi_n$ be an index of aggregate queries\footnote{Our omission of the word ``simple'' here is intentional: each \smash{$\oldPi_{\j}$} can either be simple index of aggregate queries or one of the more sophisticated types we introduce soon. In particular, by allowing some or all of the \smash{$\oldPi_{\j}$} to be different kinds of indexes of aggregate queries, we can use \definitionref{def:tprivacy:aggregate} to define privacy for all constructions in the sequel.} for $\D$. Requests are \textsl{$\t$-private with respect to $\oldPi_1,\ldots,\oldPi_n$} if, for every coalition $\coalition\subseteq\ival{\ell}$ of at most $\t$ servers, for every record index $i\in\ival{\p}$, and for every index of aggregate queries $\oldPi\in\{\oldPi_1,\ldots,\oldPi_n\}$,
\begin{align*}
    \Pr\bigl[I=i\bigm\vert \Query[\coalition]=(\oldPi\semicolon\vecQ[\j_1],\ldots,\vecQ[\j_{\t}])\bigr]&=\Pr\bigl[I=i\bigm\vert E_{\oldPi}\bigr],
\end{align*}
where $I$ and $\Query[\coalition]$ denote the random variables respectively describing the ``category'' index the user requests and the joint distribution of query vectors it sends to servers in $\coalition$ (including the ``hint'' that the query should go through $\oldPi$), and where $E_{\oldPi}$ is the event that the request is through $\oldPi$.
\end{definition}

From this definition, we understand that we can replace any ``index of queries'' matrices in any observations, definitions, and theories with the ``index of aggregate queries'' so far we studied in this chapter. For example, \theoremref{THM:UARY} turns into\emdash

\begin{theorem}\label{THM:UARY:aggregate}
Fix $\u>1$ and $j\in\ival[0]{\u-1}$, and let $\oldPi=\bigl(\oldPi_1,\ldots,\oldPi_{\ell}\bigr)\in\bigl(\F^{\pbyr}\bigr){}^{\ell}$ be buckets of a $\u$-batch index of aggregate queries with bucket coordinates $\x[1],\ldots,\x[\ell]\in\F\setminus\{0,\ldots,\u-1\}$. If \smash{$(\x[1],\vecQ[\j_1]),\ldots,(\x[\ell],\vecQ[\j_{\ell}])$} is a sequence of component-wise $(\t+1,\ell)\mkern2mu$-threshold shares of a standard basis vector $\e[]\in\F^{\p}$ encoded at $x=j$, then \smash{$(\oldPi,\x[1],\vecQ[\j_1]),\ldots,(\oldPi,\x[\ell],\vecQ[\j_{\ell}])$} is $\t$-private with respect to $\oldPi$.
\end{theorem}

Where we define $\u$-batch index of aggregate queries as follows\emdash

\begin{definition}\label{def:batchindex:aggregate}
Fix $\u>1$ and let $\x[1],\ldots,\x[\ell]\in\F\setminus\{0\mkern0.5mu,\ldots,\u-1\}$ be pairwise distinct scalars. 
A sequence $\oldPi_1,\ldots,\oldPi_{\ell}\in\F^{\pbyr}$ of matrices is a \textsl{$\u$-batch index of aggregate queries} for Goldberg's IT-PIR with bucket coordinates $\x[1],\ldots,\x[\ell]$ if (i)~$\oldPi_{i_1}\neq\oldPi_{i_2}$ for some $i_1,i_2\in\ival{\ell}$, and (ii)~for each $j=0\mkern1.5mu,\ldots,\u-1$,
\begin{align*}
\pi_j\coloneqq\nsum[1.35]_{i=1}^{\ell}\oldPi_i\cdot
\text{\larger[0.5]$\displaystyle\bigl(\tfrac{j\mkern3mu-\mkern3mux_1}{x_i\mkern3mu-\mkern3mux_1}\bigr)\cdots\bigl(\tfrac{j\mkern3mu-\mkern3mux_{i-1}}{x_i\mkern3mu-\mkern3mux_{i-1}}\bigr)\bigl(\tfrac{j\mkern3mu-\mkern3mux_{i+1}}{x_i\mkern3mu-\mkern3mux_{i+1}}\bigr)\cdots\bigl(\tfrac{j\mkern3mu-\mkern3mux_{\ell}}{x_i\mkern3mu-\mkern3mux_{\ell}}\bigr)$}
\end{align*}
is a simple index of aggregate queries.
\end{definition}
\begin{figure*}[t]
\begin{center}
% \begin{minipage}{0.8\textwidth}
\begin{align*}\tabcolsep=4pt\phantom{\D\coloneqq}&\left.~{\color{gray!90!black}
\begin{tabular}{p{2.5cm}p{2.5cm}p{1cm}p{1cm}p{1.5cm}p{4cm}}
\textsmaller{\texttt{author}}&
\textsmaller{\texttt{keywords}}&
\textsmaller{\texttt{year}}&
\textsmaller{\texttt{\#cites}}&
\textsmaller{\texttt{\#downloads}}&
\textsmaller{\texttt{paper title}}\\
\end{tabular}}\right.\\[-1.35ex]
\D\coloneqq&\left\lgroup
\begin{tabular}{p{2.5cm}p{2.5cm}p{1cm}p{1cm}p{1.5cm}p{4cm}}
Syed Hafiz & PIR, MPC & 2020 & 19 & 121 & A bit more than a bit\rlap{\ldots}\\%[-0.35ex]
Syed Hafiz & MPC, DPF & 2020 & 77 & 911 & A scanning-free learn\rlap{\ldots}\\%[-0.35ex]
Ryan Henry & DPF & 2020 & 31 & 642 & Polynomical batch\rlap{\ldots}\\%[-0.35ex]
Syed Hafiz & PIR, DPF & 2019 & 7 & 312 & Querying for queries\rlap{\ldots}\\%[-0.35ex]
Ryan Henry & DPF, PIR & 2019 & 53 & 59 & There are 10 types\rlap{\ldots}\\%[-0.35ex]
Ryan Henry & MPC, PIR & 2019 & 17 & 19 & Pirsona: recommend\rlap{\ldots}\\
\end{tabular}\right\rgroup~\\
\end{align*}
% \end{minipage}
\caption[Toy example of an ePrint database comprising six papers and metadata.]{Toy example of an ePrint database comprising six papers and associated metadata.\label{fig:expressive:eprint}}
\end{center}
\end{figure*}
\subsection{Example application: Private aggregate queries over an ePrint archive}
We realize how the indexes of aggregate queries do fascinating expressive queries privately by another toy example illustrated in \figureref{fig:expressive:eprint}. The ePrint archive $\D$ holds six papers stored in the order they are published on the site. Each record of $\D$ corresponds to one paper and its schema includes the attributes of \texttt{author} name, \texttt{keywords}, \texttt{year} of publication, citation counts \texttt{\#cites}, number of downloads \texttt{\#downloads}, and $\texttt{paper title}$. Note that this schema has only two numerical fields on which a PIR client can make the private aggregate query. 

Suppose we target to build a PIR set up to support aggregate queries like ``total citations and downloads of papers of a given author on a given keyword in the last two years.'' To facilitate such interesting (but complicated and) aggregate queries, we need two simple indexes of aggregate queries as follows:
\begin{align*}
% \arraycolsep=3pt
\Pi[PIR]\coloneqq\left\lgroup\!\begin{array}{lllllll}
\color{gray!90!black}{\fontsize{7}{7}\selectfont \texttt{(@Syed Hafiz)}}&1&0&0&1&0&0\\%[-0.25ex]
\color{gray!90!black}{\fontsize{7}{7}\selectfont \texttt{(@Ryan Henry)}}&0&0&0&0&0&1%[-0.25ex]
\end{array}\!\right\rgroup
\text{ and\, }
\Pi[DPF]\coloneqq\left\lgroup\!\begin{array}{llllllll}
\color{gray!90!black}{\fontsize{7}{7}\selectfont \texttt{(@Syed Hafiz)}}&0&1&0&1&0&0\\%[-0.25ex]
\color{gray!90!black}{\fontsize{7}{7}\selectfont \texttt{(@Ryan Henry)}}&0&0&1&0&1&0%[-0.25ex]
\end{array}\!\right\rgroup
\end{align*}
Each row of $\Pi[PIR]$ and $\Pi[DPF]$ is a standard aggregate query that is pointing to the papers published in the last two years on a particular keyword. For instance, the second row of $\Pi[DPF]$ adds the values of numeric attributes (e.g., \texttt{\#cites} and \texttt{\#downloads}) of two papers that are published in the last two years and have ``DPF'' in their \texttt{keywords} list. Now we can batch them by the process of \sectionref{ss:expressive:2batch}, i.e., the 2-ary polynomial batch codes, and produce:
\begin{align*}
% \arraycolsep=3pt
\Pi[PIR,DPF](x) \coloneqq\left\lgroup\!\begin{array}{cccccc}
1-x &   x   &   0   &   1   &   0   &   0\\%[-0.35ex]
0   &   0   &   x   &   0   &   1   &   1-x
\end{array}\!\right\rgroup\in\bigl(\F[x]\bigr)^{2\times6}.
\end{align*}
We can easily check that evaluating $\Pi[PIR,DPF](x)$ component-wise at $x=0$ and $x=1$ recovers $\Pi[PIR]$ and $\Pi[DPF]$, respectively. Each of $\ell$ servers holds an evaluation of $\Pi[PIR,DPF](x)$ at $x=\x$, where $\x[1],\ldots,\x[\ell]\in\F\setminus\{0\mkern0.5mu,\mkern-1mu1\}$ are arbitrary, pairwise distinct scalars. (Note that each such evaluation, a bucket held by a server, is a $2$-batch index of aggregate queries per \definitionref{def:batchindex:aggregate}.) If the client likes to know total citations and downloads of papers of \emph{Ryan Henry} on \emph{PIR} in the last two years, she encodes the standard basis vector $\e[1]\in\F^2$ at $x=0$. Likewise, if she wants to fetch total citations and downloads of papers of \emph{Ryan Henry} on \emph{DPF} in the last two years, she encodes the standard basis vector $\e[1]\in\F^2$ at $x=1$ in a different query. Moreover, according to \sectionref{ss:expressive:indexbatch}, we can enable the client to fetch aggregate information of both of them only in a single round by the batch query mechanism. In that case, she has to encode the same standard basis vector $\e[1]$ at $x=0$ and $x=1$ at once. This aggregate query brings the information of total citations and downloads of papers of \emph{Ryan Henry} on \emph{PIR} and \emph{DPF} in the last two years, respectively.\footnote{Note that to facilitate aggregate queries, the service provider projects on two columns (corresponds to numeric attributes \texttt{\#cites} and \texttt{\#downloads}) from the entire database and conceptualize a \emph{thin} database on what the PIR computations occur at the server-side.} Thus, we can define the indexes of $k$-batch aggregate queries as follows:

\begin{definition}\label{def:indexbatch:aggregate}
Fix $k>1$ and let $\x[1],\ldots,\x[\ell]\in\F\setminus\{0\mkern0.5mu,\ldots,k-1\}$ be pairwise distinct scalars. A sequence $\oldPi_1,\ldots,\oldPi_{\ell}\in\F^{\pbyr}$ of matrices is an \textsl{index of $k$-batch aggregate queries} for Goldberg's IT-PIR with bucket coordinates $\x[1],\ldots,\x[\ell]$ if, for each $i=1,\ldots,\p$, the matrix
% \vspace*{-0.25ex}
\begin{align*}
    \left\lgroup\ensuremath{\!\!\!\begin{array}{c}\\[-3ex]\pi_{i0}\\[-0.75ex]\vdots\\[-0.25ex]\pi_{i(k-1)}\\[0.25ex]\end{array}\!\!\!}\right\rgroup
\end{align*}
% \vspace*{-0.25ex}
is a simple index of aggregate queries matrix, where, for each $j\in\ival[0]{k-1}$,
%\noindent\scalebox{0.925}[1]{~~\begin{minipage}{\columnwidth}
\begin{align*}
\pi_{ij}\coloneqq\e\mkern-1.5mu\cdot\mkern-3.5mu\nsum[1.35]_{n=1}^{\ell}\mkern-1.5mu\oldPi_n\cdot\text{\larger[0.5]$\displaystyle\bigl(\mkern-0.5mu\tfrac{j\mkern1mu-\mkern2mux_1}{x_n\mkern1.5mu-\mkern1.5mux_1}\mkern-0.5mu\bigr)\mkern-1.5mu\cdots\mkern-1.5mu\bigl(\mkern-0.5mu\tfrac{j\mkern1mu-\mkern2mux_{n-1}}{x_n\mkern1.5mu-\mkern1.5mux_{n-1}}\mkern-0.5mu\bigr)\mkern-1mu\bigl(\mkern-0.5mu\tfrac{j\mkern1mu-\mkern2mux_{n+1}}{x_n\mkern1.5mu-\mkern1.5mux_{n+1}}\mkern-0.5mu\bigr)\mkern-1.5mu\cdots\mkern-1.5mu\bigl(\mkern-0.5mu\tfrac{j\mkern1mu-\mkern2mux_{\ell}}{x_n\mkern1.5mu-\mkern1.5mux_{\ell}}\mkern-0.5mu\bigr)$}.
\end{align*}
%\end{minipage}}
\end{definition}


==> sec-ndss-review.tex <==
\newpage
\section{Revisions to NDSS 2024 reviews}\label{s:apndx:ndss2024reviews}
\subsection{Mandatory tasks}
\noindent\textbf{Plan of actions for each point}
\begin{itemize}
    \item Accumulate (verbatim) reviews related to the point
    \item Start with Syed's rebuttal response
    \item Beef up Syed's response so that all review issues are addressed
    \item Add references for any claims
\end{itemize}
\textbf{Sixteen points}
\begin{enumerate}
    \item Implications of database, client query, and IAQ changes (e.g., additions, deletions, etc.).
    \item A clearer explanation of the results obtained to compare the PAQ protocol against the baseline Goldberg's IT-PIR protocol.
    \item A clearer explanation of (CPU/GPU) machines used for different steps of the protocol.
    \item Incorporation of an apple-to-apple comparison with Splinter[7]'s Yelp case study.
    \item Motivation and practicality of multi-server IT-PIR.
    \item Minimum configuration of our protocol.
    \item Mathematical proof of security of our protocol.
    \item Explanation of extendability of our protocol from honest-but-curious (or passive) adversary model to active/malicious adversary model, aka Byzantine robustness.
    \item Discussion of the choice of a varying number of records, where each record is thin.
    \item Discussion of ethical concerns related to Tweet scraping.
    \item Modify the initial part of the paper to explicate the key idea of the protocol early.
    \item Discussion of the relation and comparison between PIR and Oblivious RAM and DB.
    \item Removing extra fats from the introduction and conclusion.
    \item Publishing open source codes.
    \item Evaluate the performance of multiplication between a client query vector and the sparse IAQ matrix on the CPU. 
    \item Experiment with thicker records.
    % \item Regenerate the (benchmarking) graphs with non-log scales.
\end{enumerate}
\subsection{Overlooked tasks}
\begin{enumerate}    
    \item Carefully go over each review to ensure that we address any smaller odds and ends brought up by reviewers.    
\end{enumerate}
